Skeptic: Automatic, Justified and Privacy-Preserving Password Composition Policy Selection

The choice of password composition policy to enforce on a password-protected system represents a critical security decision, and has been shown to significantly affect the vulnerability of user-chosen passwords to guessing attacks. In practice, however, this choice is not usually rigorous or justifiable, with a tendency for system administrators to choose password composition policies based on intuition alone. In this work, we propose a novel methodology that draws on password probability distributions constructed from large sets of real-world password data which have been filtered according to various password composition policies. Password probabilities are then redistributed to simulate different user password reselection behaviours in order to automatically determine the password composition policy that will induce the distribution of user-chosen passwords with the greatest uniformity, a metric which we show to be a useful proxy to measure overall resistance to password guessing attacks. Further, we show that by fitting power-law equations to the password probability distributions we generate, we can justify our choice of password composition policy without any direct access to user password data. Finally, we present Skeptic -- a software toolkit that implements this methodology, including a DSL to enable system administrators with no background in password security to compare and rank password composition policies without resorting to expensive and time-consuming user studies. Drawing on 205,176,321 pass words across 3 datasets, we lend validity to our approach by demonstrating that the results we obtain align closely with findings from a previous empirical study into password composition policy effectiveness.

==> _appendices.tex <==
\section{Experimental data: Shay et al.}
The following results were produced for each dataset. Rankings produced by Skeptic under each selection mode (heading ``Skeptic'') are compared to those by Shay et al. \cite{shay2016designing} (heading ``Shay'') at $10^{14}$ guesses. Power-law curve $\alpha$ values given (heading ``$\alpha$'', as well as distance between our rankings and previous results (heading ``Distance''). Mean pairwise ranking distance ($mprd$) is given for each to give an idea of overall agreement and is computed by averaging the distance column.

\subsection{Yahoo}
The following results produced by Pyrrho from the Yahoo dataset. 

\begin{table}[H] \label{tbl:a-yahoo-prop}
\centering
\caption{Policy rankings produced under proportional reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.15000 & 0        \\ \hline % -0.150000001833355
basic20  & 2    & 3       & -0.22732 & 1        \\ \hline % -0.22731830236841
2word16  & 3    & 2       & -0.18900 & 1        \\ \hline % -0.188997503044491
basic16  & 4    & 7       & -0.45304 & 3        \\ \hline % -0.45303574888882
3class12 & 5    & 4       & -0.28309 & 1        \\ \hline % -0.283097964529562
2word12  & 6    & 6       & -0.31745 & 0        \\ \hline % -0.317451317379454
comp8    & 7    & 5       & -0.29652 & 2        \\ \hline % -0.296523485604993
basic12  & 8    & 8       & -0.47954 & 0        \\ \hline % -0.479541875046041
\end{tabular}
\begin{equation*}
    mprd=1
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under convergent reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 7       & -1.33182 & 6        \\ \hline % -1.3318152699160488
basic20  & 2    & 8       & -1.65587 & 6        \\ \hline % -1.6558723484160862
2word16  & 3    & 6       & -1.33178 & 3        \\ \hline % -1.3317786933594493
basic16  & 4    & 5       & -1.02369 & 1        \\ \hline % -1.0236920667679512
3class12 & 5    & 2       & -0.77450 & 3        \\ \hline % -0.7745013924378557
2word12  & 6    & 3       & -0.82019 & 3        \\ \hline % -0.8201873276216698
comp8    & 7    & 4       & -0.87005 & 3        \\ \hline % -0.8700493666798914
basic12  & 8    & 1       & -0.77239 & 7        \\ \hline % -0.7723873654120519
\end{tabular}
\begin{equation*}
    mprd=4
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under extraneous reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.04211 & 0        \\ \hline % -0.04210526402632619
basic20  & 2    & 4       & -0.05134 & 2        \\ \hline % -0.05134151255309264
2word16  & 3    & 2       & -0.05134 & 1        \\ \hline % -0.05134151255309264
basic16  & 4    & 6       & -0.17558 & 2        \\ \hline % -0.17558403806147313
3class12 & 5    & 5       & -0.15869 & 0        \\ \hline % -0.15869415660817537
2word12  & 6    & 7       & -0.18670 & 1        \\ \hline % -0.18670016935807232
comp8    & 7    & 3       & -0.15048 & 4        \\ \hline % -0.15048415667165857
basic12  & 8    & 8       & -0.35504 & 0        \\ \hline % -0.35504148566217963
\end{tabular}
\begin{equation*}
    mprd=1.25
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under null reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.00016 & 0        \\ \hline % -0.00015790845114059846
basic20  & 2    & 2       & -0.00017 & 0        \\ \hline % -0.0001748125629368484
2word16  & 3    & 3       & -0.00034 & 0        \\ \hline % -0.0003444676692301792
basic16  & 4    & 6       & -0.01238 & 2        \\ \hline % -0.012379177947589803
3class12 & 5    & 5       & -0.00946 & 0        \\ \hline % -0.009464853216191964
2word12  & 6    & 7       & -0.01360 & 1        \\ \hline % -0.013602453430650915
comp8    & 7    & 4       & -0.00620 & 3        \\ \hline % -0.006197599482015045
basic12  & 8    & 8       & -0.16874 & 0        \\ \hline % -0.16874098618285094
\end{tabular}
\begin{equation*}
    mprd=0.75
\end{equation*}
\end{table}

\subsection{RockYou}
The following results produced by Pyrrho from the RockYou dataset.

\begin{table}[H]
\centering
\caption{Policy rankings produced under proportional reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.32803 & 0        \\ \hline % -0.328031837920168
basic20  & 2    & 4       & -0.45407 & 2        \\ \hline % -0.454074299827686
2word16  & 3    & 3       & -0.43460 & 0        \\ \hline % -0.434602888404911
basic16  & 4    & 7       & -0.57962 & 3        \\ \hline % -0.579615909000248
3class12 & 5    & 2       & -0.33753 & 3        \\ \hline % -0.337533847665868
2word12  & 6    & 5       & -0.49108 & 1        \\ \hline % -0.491081508483271
comp8    & 7    & 6       & -0.54964 & 1        \\ \hline % -0.549638759867585
basic12  & 8    & 8       & -0.58639 & 0        \\ \hline % -0.586394707428606
\end{tabular}
\begin{equation*}
    mprd=1.25
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under convergent reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 2       & -0.73706 & 1        \\ \hline % -0.7370600303865892
basic20  & 2    & 7       & -0.86310 & 5        \\ \hline % -0.8631044205311791
2word16  & 3    & 5       & -0.79623 & 2        \\ \hline % -0.7962302362383675
basic16  & 4    & 6       & -0.85714 & 2        \\ \hline % -0.8571363235418632
3class12 & 5    & 1       & -0.66272 & 4        \\ \hline % -0.6627194044723481
2word12  & 6    & 3       & -0.74833 & 3        \\ \hline % -0.7483331444938627
comp8    & 7    & 8       & -0.92870 & 1        \\ \hline % -0.9286992229097784
basic12  & 8    & 4       & -0.77957 & 4        \\ \hline % -0.7795740115228937
\end{tabular}
\begin{equation*}
    mprd=2.75
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under extraneous reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.17322 & 0        \\ \hline % -0.1732211425958675
basic20  & 2    & 3       & -0.24107 & 1        \\ \hline % -0.241065664695532
2word16  & 3    & 4       & -0.24636 & 1        \\ \hline % -0.24636409010032567
basic16  & 4    & 7       & -0.38191 & 3        \\ \hline % -0.3819146716743862
3class12 & 5    & 2       & -0.22171 & 3        \\ \hline % -0.22171184178758788
2word12  & 6    & 6       & -0.35128 & 0        \\ \hline % -0.3512831245013512
comp8    & 7    & 5       & -0.29032 & 2        \\ \hline % -0.29031771828970143
basic12  & 8    & 8       & -0.49859 & 0        \\ \hline % -0.49858696194583363
\end{tabular}
\begin{equation*}
    mprd=1.25
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under null reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 1       & -0.00481 & 0        \\ \hline % -0.004809677968672
basic20  & 2    & 2       & -0.00774 & 0        \\ \hline % -0.007736129787373
2word16  & 3    & 3       & -0.01311 & 0        \\ \hline % -0.013105260705404
basic16  & 4    & 7       & -0.11203 & 3        \\ \hline % -0.112034361640235
3class12 & 5    & 5       & -0.01818 & 0        \\ \hline % -0.018181608224376
2word12  & 6    & 6       & -0.07942 & 0        \\ \hline % -0.079421729135592
comp8    & 7    & 4       & -0.01573 & 3        \\ \hline % -0.015733457331725
basic12  & 8    & 8       & -0.32090 & 0        \\ \hline % -0.320900187849602
\end{tabular}
\begin{equation*}
    mprd=0.75
\end{equation*}
\end{table}

\subsection{LinkedIn}
The following results produced by Pyrrho from the LinkedIn dataset. 

\begin{table}[H]
\centering
\caption{Policy rankings produced under proportional reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 2       & -0.45101 & 1        \\ \hline % -0.4510142240235451
basic20  & 2    & 1       & -0.45052 & 1        \\ \hline % -0.4505241513185305
2word16  & 3    & 3       & -0.52490 & 0        \\ \hline % -0.5248958537542961
basic16  & 4    & 4       & -0.57100 & 0        \\ \hline % -0.5709974791941261
3class12 & 5    & 5       & -0.58018 & 0        \\ \hline % -0.5801754605463195
2word12  & 6    & 7       & -0.61491 & 1        \\ \hline % -0.6149086458490779
comp8    & 7    & 8       & -0.65135 & 1        \\ \hline % -0.6513514086846621
basic12  & 8    & 6       & -0.59159 & 2        \\ \hline % -0.59158613933814
\end{tabular}
\begin{equation*}
    mprd=0.75
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under convergent reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 5       & -0.84807 & 4        \\ \hline % -0.8480745130620257
basic20  & 2    & 8       & -0.90303 & 6        \\ \hline % -0.9030320987318488
2word16  & 3    & 7       & -0.89905 & 4        \\ \hline % -0.899054755355177
basic16  & 4    & 3       & -0.79663 & 1        \\ \hline % -0.7966304699343845
3class12 & 5    & 2       & -0.77998 & 3        \\ \hline % -0.7799770935688873
2word12  & 6    & 4       & -0.83476 & 2        \\ \hline % -0.8347560109312953
comp8    & 7    & 6       & -0.84855 & 1        \\ \hline % -0.8485486697681716
basic12  & 8    & 1       & -0.73119 & 7        \\ \hline % -0.7311926960896533
\end{tabular}
\begin{equation*}
    mprd=3.5
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under extraneous reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 2       & -0.25849 & 1        \\ \hline % -0.258487667311501
basic20  & 2    & 1       & -0.24783 & 1        \\ \hline % -0.2478302856974191
2word16  & 3    & 3       & -0.29777 & 0        \\ \hline % -0.2977719578887627
basic16  & 4    & 4       & -0.40212 & 0        \\ \hline % -0.4021997188377
3class12 & 5    & 6       & -0.43334 & 1        \\ \hline % -0.43333756896014186
2word12  & 6    & 5       & -0.42870 & 1        \\ \hline % -0.4286963998704655
comp8    & 7    & 7       & -0.45946 & 0        \\ \hline % -0.4594561194976184
basic12  & 8    & 8       & -0.53008 & 0        \\ \hline % -0.5300844001874699
\end{tabular}
\begin{equation*}
    mprd=0.5
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Policy rankings produced under null reselection.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Shay & Skeptic & $\alpha$ & Distance \\ \hline
3class16 & 1    & 2       & -0.00512 & 1        \\ \hline % -0.005119700140876735
basic20  & 2    & 1       & -0.00207 & 1        \\ \hline % -0.002065442726884162
2word16  & 3    & 3       & -0.01272 & 0        \\ \hline % -0.01271757597379048
basic16  & 4    & 4       & -0.11099 & 0        \\ \hline % -0.11099256296522678
3class12 & 5    & 6       & -0.18384 & 1        \\ \hline % -0.1838419851528793
2word12  & 6    & 5       & -0.17379 & 1        \\ \hline % -0.17379245774700025
comp8    & 7    & 7       & -0.21988 & 0        \\ \hline % -0.2198828897383922
basic12  & 8    & 8       & -0.44626 & 0        \\ \hline % -0.44625701958531794
\end{tabular}
\begin{equation*}
    mprd=0.5
\end{equation*}
\end{table}

\section{Replication results: Shay et al.}
The following scatter plots show the correlation between the $\alpha$ values of power-law equations fitted to proportional (average case) reselection results produced by \textit{Skeptic} and the rankings empirically determined by Shay et al. in \cite{shay2016designing}. Each plot is annotated with its Pearson correlation coefficient $\rho$.

\subsection{Yahoo}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/pdf/yahoo_shay_alpha_corr.pdf}
    \caption{Proportional reselection.}
    \label{fig:my_label_1}
    \begin{equation*}
        \rho=-0.7128752913482401
    \end{equation*}
\end{figure}

\subsection{RockYou}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/pdf/rockyou_shay_alpha_corr.pdf}
    \caption{Proportional reselection.}
    \label{fig:my_label_2}
    \begin{equation*}
        \rho=-0.6384628682993778
    \end{equation*}
\end{figure}

\subsection{LinkedIn}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\columnwidth]{figures/pdf/linkedin_shay_alpha_corr.pdf}
    \caption{Proportional reselection.}
    \label{fig:my_label_3}
    \begin{equation*}
        \rho=-0.9005449627393818
    \end{equation*}
\end{figure}

\section{Experimental data: Weir et al.}

\begin{table}[H]
\centering
\caption{Yahoo proportional}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 2       & -0.32002 & 1        \\ \hline % -0.320019090237718
symbol9  & 2    & 1       & -0.29548 & 1        \\ \hline % -0.295475843288516
symbol8  & 3    & 7       & -0.35748 & 4        \\ \hline % -0.357477064159878
upper10  & 4    & 5       & -0.33300 & 1        \\ \hline % -0.332996715456861
symbol7  & 5    & 8       & -0.41519 & 3        \\ \hline % -0.415192888759335
upper9   & 6    & 4       & -0.33151 & 2        \\ \hline % -0.331512666495103
upper8   & 7    & 6       & -0.34709 & 1        \\ \hline % -0.34708686659925
upper7   & 8    & 3       & -0.32624 & 5        \\ \hline % -0.326237545968052
basic10  & 9    & 9       & -0.48500 & 0        \\ \hline % -0.485004346203473
basic9   & 10   & 10      & -0.49911 & 0        \\ \hline % -0.499108167959326
basic8   & 11   & 12      & -0.56605 & 1        \\ \hline % -0.566051941104415
basic7   & 12   & 11      & -0.56231 & 1        \\ \hline % -0.562306050086818
\end{tabular}
\begin{equation*}
    mprd=1.67 % 1.66666666666667
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Yahoo convergent}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 12      & -0.81123 & 11       \\ \hline % -0.811227798800374
symbol9  & 2    & 8       & -0.72096 & 6        \\ \hline % -0.720963029089251
symbol8  & 3    & 10      & -0.76600 & 7        \\ \hline % -0.765999572114918
upper10  & 4    & 9       & -0.75269 & 5        \\ \hline % -0.752686181848347
symbol7  & 5    & 11      & -0.78870 & 6        \\ \hline % -0.788700654817024
upper9   & 6    & 4       & -0.68842 & 2        \\ \hline % -0.688419067420068
upper8   & 7    & 6       & -0.70280 & 1        \\ \hline % -0.702796687770826
upper7   & 8    & 1       & -0.63983 & 7        \\ \hline % -0.63983100467906
basic10  & 9    & 7       & -0.70883 & 2        \\ \hline % -0.708832661734246
basic9   & 10   & 3       & -0.67839 & 7        \\ \hline % -0.678388765092003
basic8   & 11   & 5       & -0.69848 & 6        \\ \hline % -0.698480480512314
basic7   & 12   & 2       & -0.66790 & 10       \\ \hline % -0.667901363570134
\end{tabular}
\begin{equation*}
    mprd=5.83 % 5.83333333333333
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Yahoo extraneous}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 1       & -0.18744 & 0        \\ \hline % -0.187442966703073
symbol9  & 2    & 2       & -0.19155 & 0        \\ \hline % -0.19154796592903
symbol8  & 3    & 4       & -0.23556 & 1        \\ \hline % -0.23555861985848
upper10  & 4    & 3       & -0.22055 & 1        \\ \hline % -0.220554417524206
symbol7  & 5    & 8       & -0.27091 & 3        \\ \hline % -0.270907280037943
upper9   & 6    & 5       & -0.24554 & 1        \\ \hline % -0.245536024258508
upper8   & 7    & 6       & -0.26689 & 1        \\ \hline % -0.266894897049293
upper7   & 8    & 7       & -0.26689 & 1        \\ \hline % -0.266894897049293
basic10  & 9    & 9       & -0.43376 & 0        \\ \hline % -0.43376475498875
basic9   & 10   & 10      & -0.47508 & 0        \\ \hline % -0.475078293960674
basic8   & 11   & 11      & -0.54362 & 0        \\ \hline % -0.543615417117954
basic7   & 12   & 12      & -0.56231 & 0        \\ \hline % -0.562306050881446
\end{tabular}
\begin{equation*}
    mprd=0.67 % 0.666666666666667
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{Yahoo null}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 1       & -0.01556 & 0        \\ \hline % -0.015564167473273
symbol9  & 2    & 2       & -0.01887 & 0        \\ \hline % -0.018871220622022
symbol8  & 3    & 4       & -0.03759 & 1        \\ \hline % -0.037592310964835
upper10  & 4    & 3       & -0.03321 & 1        \\ \hline % -0.033205695796485
symbol7  & 5    & 6       & -0.06282 & 1        \\ \hline % -0.062818164211923
upper9   & 6    & 5       & -0.05096 & 1        \\ \hline % -0.050956596285808
upper8   & 7    & 8       & -0.08789 & 1        \\ \hline % -0.087885338307444
upper7   & 8    & 7       & -0.08667 & 1        \\ \hline % -0.086671352731622
basic10  & 9    & 9       & -0.32446 & 0        \\ \hline % -0.324458546763458
basic9   & 10   & 10      & -0.39767 & 0        \\ \hline % -0.397667944294436
basic8   & 11   & 11      & -0.52440 & 0        \\ \hline % -0.524401090971686
basic7   & 12   & 12      & -0.54077 & 0        \\ \hline % -0.540768194296323
\end{tabular}
\begin{equation*}
    mprd=0.5
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{RockYou proportional}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 3       & -0.55159 & 2        \\ \hline % -0.551590464244535
symbol9  & 2    & 4       & -0.58810 & 2        \\ \hline % -0.588098630934787
symbol8  & 3    & 7       & -0.61414 & 4        \\ \hline % -0.61413717745509
upper10  & 4    & 1       & -0.51254 & 3        \\ \hline % -0.51253601635051
symbol7  & 5    & 5       & -0.60034 & 0        \\ \hline % -0.600338690489993
upper9   & 6    & 2       & -0.55140 & 4        \\ \hline % -0.551404671084113
upper8   & 7    & 8       & -0.61888 & 1        \\ \hline % -0.618883001691848
upper7   & 8    & 6       & -0.60294 & 2        \\ \hline % -0.60293509146904
basic10  & 9    & 9       & -0.67358 & 0        \\ \hline % -0.673580606619615
basic9   & 10   & 10      & -0.74060 & 0        \\ \hline % -0.74059964193201
basic8   & 11   & 11      & -0.75840 & 0        \\ \hline % -0.75839599758178
basic7   & 12   & 12      & -0.76364 & 0        \\ \hline % -0.763643560370707
\end{tabular}
\begin{equation*}
    mprd=1.5
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{RockYou convergent}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 6       & -0.80188 & 5        \\ \hline % -0.801875957547684
symbol9  & 2    & 4       & -0.79545 & 2        \\ \hline % -0.795454891822942
symbol8  & 3    & 8       & -0.82135 & 5        \\ \hline % -0.821354821404331
upper10  & 4    & 1       & -0.78038 & 3        \\ \hline % -0.780381961709881
symbol7  & 5    & 7       & -0.80743 & 2        \\ \hline % -0.807434593778842
upper9   & 6    & 2       & -0.78159 & 4        \\ \hline % -0.781585945960103
upper8   & 7    & 9       & -0.82309 & 2        \\ \hline % -0.823085069851623
upper7   & 8    & 3       & -0.78834 & 5        \\ \hline % -0.788341785033446
basic10  & 9    & 5       & -0.79945 & 4        \\ \hline % -0.799454426413728
basic9   & 10   & 10      & -0.82980 & 0        \\ \hline % -0.829804401209344
basic8   & 11   & 12      & -0.83558 & 1        \\ \hline % -0.8355842499383
basic7   & 12   & 11      & -0.83373 & 1        \\ \hline % -0.833734273371648
\end{tabular}
\begin{equation*}
    mprd=2.83 % 2.83333333333333
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{RockYou extraneous}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 2       & -0.40493 & 1        \\ \hline % -0.404927724373475
symbol9  & 2    & 4       & -0.46072 & 2        \\ \hline % -0.460721818409071
symbol8  & 3    & 5       & -0.48545 & 2        \\ \hline % -0.48544869139838
upper10  & 4    & 1       & -0.38164 & 3        \\ \hline % -0.381636077778196
symbol7  & 5    & 6       & -0.48818 & 1        \\ \hline % -0.488184082776828
upper9   & 6    & 3       & -0.44141 & 3        \\ \hline % -0.441409632719588
upper8   & 7    & 7       & -0.50596 & 0        \\ \hline % -0.505961148926222
upper7   & 8    & 8       & -0.52077 & 0        \\ \hline % -0.520772791592121
basic10  & 9    & 9       & -0.63137 & 0        \\ \hline % -0.631367204571857
basic9   & 10   & 10      & -0.70026 & 0        \\ \hline % -0.700264536092272
basic8   & 11   & 11      & -0.74041 & 0        \\ \hline % -0.740408621476455
basic7   & 12   & 12      & -0.74860 & 0        \\ \hline % -0.748597473549761
\end{tabular}
\begin{equation*}
    mprd=1
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{RockYou null}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 2       & -0.15407 & 1        \\ \hline % -0.154070732249245
symbol9  & 2    & 4       & -0.22450 & 2        \\ \hline % -0.224503431772083
symbol8  & 3    & 5       & -0.26824 & 2        \\ \hline % -0.268238620492176
upper10  & 4    & 1       & -0.10831 & 3        \\ \hline % -0.108305992409738
symbol7  & 5    & 6       & -0.28506 & 1        \\ \hline % -0.285056407782036
upper9   & 6    & 3       & -0.18380 & 3        \\ \hline % -0.183796249244513
upper8   & 7    & 7       & -0.29844 & 0        \\ \hline % -0.298436168527346
upper7   & 8    & 8       & -0.31507 & 0        \\ \hline % -0.315068024766683
basic10  & 9    & 9       & -0.53300 & 0        \\ \hline % -0.533001823311373
basic9   & 10   & 10      & -0.64805 & 0        \\ \hline % -0.648050289801095
basic8   & 11   & 11      & -0.70358 & 0        \\ \hline % -0.703582448186162
basic7   & 12   & 12      & -0.73241 & 0        \\ \hline % -0.732412916718902
\end{tabular}
\begin{equation*}
    mprd=1
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{LinkedIn proportional}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 2       & -0.59113 & 1        \\ \hline % -0.591125607565898
symbol9  & 2    & 1       & -0.57306 & 1        \\ \hline % -0.573062312278435
symbol8  & 3    & 3       & -0.63716 & 0        \\ \hline % -0.637160061538711
upper10  & 4    & 6       & -0.64463 & 2        \\ \hline % -0.644631998879243
symbol7  & 5    & 5       & -0.63890 & 0        \\ \hline % -0.63890220739714
upper9   & 6    & 7       & -0.64477 & 1        \\ \hline % -0.644771493436183
upper8   & 7    & 9       & -0.67203 & 2        \\ \hline % -0.672030599630624
upper7   & 8    & 8       & -0.66124 & 0        \\ \hline % -0.661240194459474
basic10  & 9    & 4       & -0.63873 & 5        \\ \hline % -0.638734067627644
basic9   & 10   & 10      & -0.68880 & 0        \\ \hline % -0.688795978953019
basic8   & 11   & 12      & -0.72456 & 1        \\ \hline % -0.724556525176091
basic7   & 12   & 11      & -0.71769 & 1        \\ \hline % -0.717691552183719
\end{tabular}
\begin{equation*}
    mprd=1.17 % 1.16666666666667
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{LinkedIn convergent}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
basic7   & 12   & 4       & -0.78039 & 8        \\ \hline % -0.780385300281843
basic8   & 11   & 7       & -0.79384 & 4        \\ \hline % -0.793844107137502
basic9   & 10   & 3       & -0.77558 & 7        \\ \hline % -0.77558016778182
basic10  & 9    & 1       & -0.74921 & 8        \\ \hline % -0.749209480818537
upper7   & 8    & 6       & -0.79011 & 2        \\ \hline % -0.790113699350695
upper8   & 7    & 11      & -0.81234 & 4        \\ \hline % -0.812340892955823
upper9   & 6    & 5       & -0.78643 & 1        \\ \hline % -0.786425446879901
symbol7  & 5    & 10      & -0.80207 & 5        \\ \hline % -0.802067042869362
upper10  & 4    & 12      & -0.81872 & 8        \\ \hline % -0.818723971577312
symbol8  & 3    & 9       & -0.80038 & 6        \\ \hline % -0.800376870527337
symbol9  & 2    & 2       & -0.75850 & 0        \\ \hline % -0.758496120268716
symbol10 & 1    & 8       & -0.79438 & 7        \\ \hline % -0.794380401470364
\end{tabular}
\begin{equation*}
    mprd=5
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{LinkedIn extraneous}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 1       & -0.45380 & 0        \\ \hline % -0.453799878840267
symbol9  & 2    & 2       & -0.46565 & 0        \\ \hline % -0.465646796670343
symbol8  & 3    & 3       & -0.51610 & 0        \\ \hline % -0.516103963611644
upper10  & 4    & 5       & -0.53186 & 1        \\ \hline % -0.531863189414612
symbol7  & 5    & 4       & -0.51839 & 1        \\ \hline % -0.518388873565154
upper9   & 6    & 6       & -0.55852 & 0        \\ \hline % -0.558521132876959
upper8   & 7    & 7       & -0.59859 & 0        \\ \hline % -0.598592761398404
upper7   & 8    & 8       & -0.60101 & 0        \\ \hline % -0.601009738020508
basic10  & 9    & 9       & -0.60275 & 0        \\ \hline % -0.602754448078005
basic9   & 10   & 10      & -0.66974 & 0        \\ \hline % -0.66973846396697
basic8   & 11   & 12      & -0.71573 & 1        \\ \hline % -0.715732913437398
basic7   & 12   & 11      & -0.71214 & 1        \\ \hline % -0.7121449144858
\end{tabular}
\begin{equation*}
    mprd=0.33 % 0.333333333333333
\end{equation*}
\end{table}

\begin{table}[H]
\centering
\caption{LinkedIn null}
\begin{tabular}{|l|l|l|l|l|}
\hline
Policy   & Weir & Skeptic & $\alpha$ & Distance \\ \hline
symbol10 & 1    & 1       & -0.23443 & 0        \\ \hline % -0.234427453587019
symbol9  & 2    & 2       & -0.26074 & 0        \\ \hline % -0.260740493970895
symbol8  & 3    & 3       & -0.35575 & 0        \\ \hline % -0.355747988006753
upper10  & 4    & 4       & -0.35737 & 0        \\ \hline % -0.357367299269786
symbol7  & 5    & 5       & -0.36453 & 0        \\ \hline % -0.364526548309825
upper9   & 6    & 6       & -0.41293 & 0        \\ \hline % -0.412934580291385
upper8   & 7    & 8       & -0.50475 & 1        \\ \hline % -0.504746418395145
upper7   & 8    & 7       & -0.49261 & 1        \\ \hline % -0.492610064748683
basic10  & 9    & 9       & -0.55796 & 0        \\ \hline % -0.557956500420314
basic9   & 10   & 10      & -0.63726 & 0        \\ \hline % -0.637258050629719
basic8   & 11   & 11      & -0.69777 & 0        \\ \hline % -0.697771266850606
basic7   & 12   & 12      & -0.70531 & 0        \\ \hline % -0.705309373511038
\end{tabular}
\begin{equation*}
    mprd=0.17 % 0.166666666666667
\end{equation*}
\end{table}








\subsubsection{Frequencies to probabilities} It is straightforward to derive a password probability distribution from the input set. If we know the frequency with which a password occurs in the input set, and the total number of passwords it contains (its \textit{magnitude}) we can straightforwardly compute the probability that that password will permit access to a randomly-selected account on the system it originated from. 
Let a password frequency record in a representation of a user credential database $D$ originating from a system supporting password characters in set $S$ be a tuple $(s \in S^*, f \in \mathbb{N}, r \in \mathbb{N})$. Here $s$ is the password, which consists of some element in the set produced by applying the Kleene star operation to $S$, $f$ is the frequency with which $s$ appears in the database, and $r$ is the rank of the password in the database when ordered by frequency (that is, the most common password would have $r=1$, the second most common $r=2$ and so on). 
% Given a record $r=(s,f)$, we write $r_s$, $r_f$, to denote the elements $s$ and $f$ respectively. For example, if $r=(\textrm{`p4ss'},100)$, then $r_s=\textrm{`p4ss'}$, and $r_f=100$. 
The magnitude $mag(D)$ of a database $D$ represents the total number of passwords present on the system, and can readily be calculated by summing the frequency of each record together.

\begin{equation*}
    mag(D) = \sum_{(s, f, r) \in D}{} f
\end{equation*}

The set of password probability records of a database $D$ can be obtained by dividing the frequency of each record by the magnitude of $D$:

\begin{equation*}
    probs(D) = \{(s, \frac{f}{mag(D)}, r)  ~|~ (s, f, r) \in D\}
\end{equation*}

We call this newly-calculated probability $p$ (i.e. the second member of tuples in the set produced by $probs$). What we are left with is a probability distribution $P$ that will map passwords $s$ (outcomes) to the probability that a randomly-selected account on the system will have that password.

\begin{equation*}
    P(s) = 
    \begin{cases}
        p       & \text{if } (s, p, r) \in probs(D)\\
        0       & \text{otherwise}
    \end{cases}
\end{equation*}

We can plot the $r$ and $p$ of each tuple in $probs(D)$ as $x$ and $y$ coordinates respectively to visualise the \textit{rank-probability distribution} of $probs(D)$. Figure~\ref{fig:yahoo-basic6-scatter} shows a scatter plot of the rank-probability distribution of the Yahoo dataset used in this study. Note the log-log axes and the extremely long tail of the distribution made up of passwords with probabilities corresponding to frequencies in the low single digits. This is characteristic of a distribution of user-chosen passwords, with few passwords chosen very often and many passwords being chosen very rarely.

\begin{figure}[ht]
    \includegraphics[width=\columnwidth]{figures/pdf/yahoo_basic6_scatter.pdf}
    \caption{A scatter plot of the rank-probability distribution of passwords in the Yahoo dataset \cite{gross2012yahoo} used in this study.}
    \label{fig:yahoo-basic6-scatter}
\end{figure}

\begin{landscape}
  \begin{table}
    \centering
    \resizebox{\columnwidth}{!}{
      \begin{tabular}[c]{|*{16}{l|}}
        \hline
        & & \multirow{2}{*}{Policy} & \multicolumn{4}{c|}{Yahoo} & \multicolumn{4}{c|}{RockYou} & \multicolumn{4}{c|}{LinkedIn}\\
      \cline{4-15}
      & & & Shay & Skeptic & $\alpha$ & Distance & Shay & Skeptic & $\alpha$ & Distance & Shay & Skeptic & $\alpha$ & Distance\\
      \hline
      \multirow{32}{*}{\rotatebox{90}{Reselection modes}} & \multirow{8}{*}{\rotatebox{90}{Null}} & 3class16 & 1 & 1 & -0.00015790845 & 0 & 1 & 1 & -0.00480967797 & 0 & 1 & 2 & -0.00511970014 & 1\\
      \cline{3-15}
      & & basic20 & 2 & 2 & -0.00017481256 & 0 & 2 & 2 & -0.00773612979 & 0 & 2 & 1 & -0.00206544273 & 1\\
      \cline{3-15}
      & & 2word16 & 3 & 3 & -0.00034446767 & 0 & 3 & 3 & -0.01310526071 & 0 & 3 & 3 & -0.01271757597 & 0\\
      \cline{3-15}
      & & basic16 & 4 & 6 & -0.01237917795 & 2 & 4 & 7 & -0.11203436164 & 3 & 4 & 4 & -0.11099256297 & 0\\
      \cline{3-15}
      & & 3class12 & 5 & 5 & -0.00946485322 & 0 & 5 & 5 & -0.01818160822 & 0 & 5 & 6 & -0.18384198515 & 1\\
      \cline{3-15}
      & & 2word12 & 6 & 7 & -0.01360245343 & 1 & 6 & 6 & -0.07942172914 & 0 & 6 & 5 & -0.17379245775 & 1\\
      \cline{3-15}
      & & comp8 & 7 & 4 & -0.00619759948 & 3 & 7 & 4 & -0.01573345733 & 3 & 7 & 7 & -0.21988288974 & 0\\
      \cline{3-15}
      & & basic12 & 8 & 8 & -0.16874098618 & 0 & 8 & 8 & -0.32090018785 & 0 & 8 & 8 & -0.44625701959 & 0\\
      \cline{2-15}
      & \multirow{8}{*}{\rotatebox{90}{Proportional}} & 3class16 & 1 & 1 & -0.15000000183 & 0 & 1 & 1 & -0.32803183792 & 0 & 1 & 2 & -0.45101422402 & 1\\
      \cline{3-15}
      & & basic20 & 2 & 3 & -0.22731830237 & 1 & 2 & 4 & -0.45407429983 & 2 & 2 & 1 & -0.45052415132 & 1\\
      \cline{3-15}
      & & 2word16 & 3 & 2 & -0.18899750304 & 1 & 3 & 3 & -0.4346028884 & 0 & 3 & 3 & -0.52489585375 & 0\\
      \cline{3-15}
      & & basic16 & 4 & 7 & -0.45303574889 & 3 & 4 & 7 & -0.579615909 & 3 & 4 & 4 & -0.57099747919 & 0\\
      \cline{3-15}
      & & 3class12 & 5 & 4 & -0.28309796453 & 1 & 5 & 2 & -0.33753384767 & 3 & 5 & 5 & -0.58017546055 & 0\\
      \cline{3-15}
      & & 2word12 & 6 & 6 & -0.31745131738 & 0 & 6 & 5 & -0.49108150848 & 1 & 6 & 7 & -0.61490864585 & 1\\
      \cline{3-15}
      & & comp8 & 7 & 5 & -0.2965234856 & 2 & 7 & 6 & -0.54963875987 & 1 & 7 & 8 & -0.65135140868 & 1\\
      \cline{3-15}
      & & basic12 & 8 & 8 & -0.47954187505 & 0 & 8 & 8 & -0.58639470743 & 0 & 8 & 6 & -0.59158613934 & 2\\
      \cline{2-15}
      & \multirow{8}{*}{\rotatebox{90}{Extraneous}} & 3class16 & 1 & 1 & -0.04210526403 & 0 & 1 & 1 & -0.1732211426 & 0 & 1 & 2 & -0.25848766731 & 1\\
      \cline{3-15}
      & & basic20 & 2 & 4 & -0.15048415667 & 2 & 2 & 3 & -0.2410656647 & 1 & 2 & 1 & -0.2478302857 & 1\\
      \cline{3-15}
      & & 2word16 & 3 & 2 & -0.05134151255 & 1 & 3 & 4 & -0.2463640901 & 1 & 3 & 3 & -0.29777195789 & 0\\
      \cline{3-15}
      & & basic16 & 4 & 6 & -0.17558403806 & 2 & 4 & 7 & -0.38191467167 & 3 & 4 & 4 & -0.40219971884 & 0\\
      \cline{3-15}
      & & 3class12 & 5 & 5 & -0.15869415661 & 0 & 5 & 2 & -0.22171184179 & 3 & 5 & 6 & -0.43333756896 & 1\\
      \cline{3-15}
      & & 2word12 & 6 & 7 & -0.18670016936 & 1 & 6 & 6 & -0.3512831245 & 0 & 6 & 5 & -0.42869639987 & 1\\
      \cline{3-15}
      & & comp8 & 7 & 3 & -0.15048415667 & 4 & 7 & 5 & -0.29031771829 & 2 & 7 & 7 & -0.4594561195 & 0\\
      \cline{3-15}
      & & basic12 & 8 & 8 & -0.35504148566 & 0 & 8 & 8 & -0.49858696195 & 0 & 8 & 8 & -0.53008440019 & 0\\
      \cline{2-15}
      & \multirow{8}{*}{\rotatebox{90}{Convergent}} & 3class16 & 1 & 7 & -1.33181526992 & 6 & 1 & 2 & -0.73706003039 & 1 & 1 & 5 & -0.84807451306 & 4\\
      \cline{3-15}
      & & basic20 & 2 & 8 & -1.65587234842 & 6 & 2 & 7 & -0.86310442053 & 5 & 2 & 8 & -0.90303209873 & 6\\
      \cline{3-15}
      & & 2word16 & 3 & 6 & -1.33177869336 & 3 & 3 & 5 & -0.79623023624 & 2 & 3 & 7 & -0.89905475536 & 4\\
      \cline{3-15}
      & & basic16 & 4 & 5 & -1.02369206677 & 1 & 4 & 6 & -0.85713632354 & 2 & 4 & 3 & -0.79663046993 & 1\\
      \cline{3-15}
      & & 3class12 & 5 & 2 & -0.77450139244 & 3 & 5 & 1 & -0.66271940447 & 4 & 5 & 2 & -0.77997709357 & 3\\
      \cline{3-15}
      & & 2word12 & 6 & 3 & -0.82018732762 & 3 & 6 & 3 & -0.74833314449 & 3 & 6 & 4 & -0.83475601093 & 2\\
      \cline{3-15}
      & & comp8 & 7 & 4 & -0.87004936668 & 3 & 7 & 8 & -0.92869922291 & 1 & 7 & 6 & -0.84854866977 & 1\\
      \cline{3-15}
      & & basic12 & 8 & 1 & -0.77238736541 & 7 & 8 & 4 & -0.77957401152 & 4 & 8 & 1 & -0.73119269609 & 7\\
      \hline
    \end{tabular}
  }
    \caption{Policy rankings under different reselection modes}
    \label{tab:comp}
  \end{table}
  \end{landscape}


==> _overview.tex <==
\jff{TBW: general description of the approach and maybe a worked-out example. The goal is for the reader to understand/get an appreciation of the contribution.
[Perhaps this section can be used to show, with a specific worked-out example, the link between reselection and PCPs ranking.]}

==> _scraps.tex <==
%%%%%
% Rankings instead of cracked password percentages: Shay et al. ($10^{14}$ guesses)
%%%%%

If we consider policy ranking instead of percentage of passwords cracked, we see a slightly stronger correlation overall, which suggests that \textit{Skeptic} is slightly more effective at password composition policy ranking than predicting the absolute resistance of password composition policies to guessing attacks. \sj{We may need to expand on this. Should we even keep this in? If we do it here we should also do it for $10^{6}$ guesses.}

\begin{table}[ht]
\caption{Pearson correlation coefficients of password policy ranks from \cite{shay2016designing} at $10^{14}$ guesses against $\alpha$-values yielded by Skeptic. Note the variation in agreement with \cite{shay2016designing} across different datasets and reselection modes.}
\begin{tabular}{|l|l|l|l|l|}
\hline
Mode         & Yahoo  & RockYou & LinkedIn & Mean   \\ \hline
% Proportional & -0.71287529134824  & -0.638462868299378 & -0.900544962739382 & -0.750627707462333 \\ \hline
Proportional & -0.713 & -0.638  & -0.901   & -0.751 \\ \hline
% Convergent   & 0.851775054641355  & -0.099557016007189 & 0.645149080376279  & 0.465789039670148  \\ \hline
Convergent   & 0.852  & -0.100  & 0.645    & 0.465  \\ \hline
% Extraneous   & -0.781421574119305 & -0.742660342463269 & -0.962768425524716 & -0.828950114035763 \\ \hline
Extraneous   & -0.781 & -0.743  & -0.963   & -0.829 \\ \hline
% Null         & -0.62934277910602  & -0.636073274291252 & -0.920578157789287 & -0.728664737062186 \\ \hline
Null         & -0.629 & -0.636  & -0.921   & -0.729 \\ \hline
\end{tabular}
\end{table}

%%%%%
% Predicate-based password compostio policy formalisms.
%%%%%

Password composition policies are enforced on different systems by a diverse range of software, which may accept password policies in different encodings. It is convenient to represent these encodings as tuples containing software configuration parameters. For example, software $A$ may take a tuple $(l \in \mathbb{N}, d \in \mathbb{N})$ where $l$ is minimum password length and $d$ is the minimum number of numeric digits a password may contain; while software $B$ might take tuples $(e \in \mathbb{Q}, w \subset S^*)$ where $e$ is the minimum Shannon entropy of the password, and $w$ is a set of prohibited passwords (a ``dictionary check''). If we wish to compare one of each of these tuples, we must first obtain them in a uniform (i.e. normalised) encoding.

To achieve this, we take advantage of the fact that any password composition policy is necessarily a predicate from $Password \rightarrow \mathbb{B}$. With this in mind, we can obtain a uniform representation of password composition policies regardless of the software they were encoded for by devising a function to decode them to a Boolean normal form. For software $A$ for example, we might devise the function in Equation~\ref{eq:norm-func-a} which will transform a password composition policy encoded for this software into a predicate in conjunctive normal form.

\begin{equation} \label{eq:norm-func-a}
    norm_A(l, d) = \lambda s. length(s) \geq l \wedge digits(s) \geq d
\end{equation}

Even though software $B$ takes a different configuration tuple, we need only specify the normalisation function in Equation~\ref{eq:norm-func-b} for tuples of this type in order to obtain a password composition policy predicate in the same representation. 

\begin{equation} \label{eq:norm-func-b}
    norm_B(e, w) = \lambda s. shannon(s) \geq e \wedge s \notin w
\end{equation}

Normalisation functions specified in this way are amenable to formal verification, not only with respect to their correctness (i.e. their conversion of software-specific configuration tuples to predicates) but also desirable properties of the predicates they generate. For instance, we can show that a policy mandating a minimum password length of 16 encoded for software $A$ as configuration tuple $(16, 0)$ and normalised to policy predicate $\phi$ confers immunity to a guessing attack consisting of passwords in an arbitrary set of guesses $G$ by showing the universal quantification in Equation~\ref{eq:simple-immunity-eg} holds.

\begin{equation} \label{eq:simple-immunity-eg}
    \phi = norm_A(16, 0) \quad\quad\quad \forall g \in G. \neg\phi(g)
\end{equation}

In the sections that follow, we use the notation $g \in \phi$ to represent the notion that $\phi(g) = \top$. \jff{The discussion above seems unnecessary. We should just say how we represent policies (at the most abstract level, since we are not using their structure in the rest of the paper). We can also introduce the notation $p \in \PCP$ to denote that a password $p$ complies with \PCP.}

In Section~\ref{subsec:authority}, we describe our implementation of \textit{Authority}, a metaprogramming utility that generates \textit{Coq} code scaffolding to streamline the process of encoding password policies as software-specific configuration tuples, normalising them to predicates and writing proofs about them, including proofs of immunity to concrete guessing attacks as in Equation~\ref{eq:simple-immunity-eg}.

%%%%%
% Ye olde self-citation.
%%%%%

Research on certified password checking \cite{ferreira2017certified} has shown that it is possible to construct ready-to-use, formally verified software that will enforce a password composition policy specified rigorously from within interactive theorem proving software. While this may grant us confidence that the password composition policy will be enforced correctly, it does not offer any such assurance that we have selected an \textit{appropriate} password composition policy for our use case.

%%%%%
% Slightly more detailed Coq immunity/vulnerability proof.
%%%%%

\begin{figure}[ht] \codeSampleFontSize
    \centering
    \begin{minted}{coq}
(* The `basic14` policy is immune to Mirai. *)
Example basic14_mirai_immune :
  immune "basic14" mirai_dict.
Proof.
  simulate.
Qed.

(* The `2class12` policy is not immune to Mirai. *)
Example _2class12_mirai_vulnerable :
  vulnerable "2class12" mirai_dict.
Proof.
  simulate.
Qed.
    \end{minted}
    \caption{Examples of two proofs in \textit{Coq}, showing that the policy named \texttt{basic14} renders a system immune to a guessing attack by the \textit{Mirai} malware, while the policy named \texttt{2class12} leaves it vulnerable.}
    \label{fig:immunity-proofs}
\end{figure}

%%%%%
% Old password rank-probability distribution paragraph.
%%%%%

We can plot the rank and probability of each password as $x$ and $y$ coordinates respectively to visualise the \textit{rank-probability distribution} over a password set. Figure~\ref{fig:yahoo-basic6-scatter} shows a scatter plot of the rank-probability distribution of the Yahoo dataset used in this study. Note the log-log axes and the extremely long tail of the distribution made up of passwords with probabilities corresponding to frequencies in the low single digits. This is characteristic of a distribution of user-chosen passwords, with few passwords chosen very often and many passwords being chosen very rarely.

\begin{figure}[ht]
    \includegraphics[width=\graphSizeMultiplier\columnwidth]{figures/pdf/yahoo_basic6_scatter.pdf}
    \caption{A scatter plot of the rank-probability distribution of passwords in the Yahoo dataset \cite{gross2012yahoo} used in this study.}
    \label{fig:yahoo-basic6-scatter}
\end{figure}

\jff{The paragraph on rank-probability distributions needs to be more motivated. Why are we mentioning it here?}
